MLModelScope: A Distributed Platform for Model Evaluation and Benchmarking at Scale

Machine Learning (ML) and Deep Learning (DL) innovations are being introduced at such a rapid pace that researchers are hard-pressed to analyze and study them. The complicated procedures for evaluating innovations, along with the lack of standard and efficient ways of specifying and provisioning ML/DL evaluation, is a major "pain point" for the community. This paper proposes MLModelScope, an open-source, framework/hardware agnostic, extensible and customizable design that enables repeatable, fair, and scalable model evaluation and benchmarking. We implement the distributed design with support for all major frameworks and hardware, and equip it with web, command-line, and library interfaces. To demonstrate MLModelScope's capabilities we perform parallel evaluation and show how subtle changes to model evaluation pipeline affects the accuracy and HW/SW stack choices affect performance.

==> Makefile <==
LATEX=pdflatex
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

SOURCES=main.tex Makefile $(shell find sections/* -type f)
FIGURES := $(shell find figs/* -type f)

all: force

.refresh:
	touch .refresh

main.pdf: main.tex .refresh $(SOURCES) $(FIGURES)
    $(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
        -pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" main

force:
	touch .refresh
	rm -fr main.pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" main

clean:
	$(LATEXMK) -C main
	rm -f main.pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" main

debug:
	$(LATEX) $(LATEXOPT) main

.PHONY: clean force once all

==> latex_figures/fig_language_cpu.tex <==


 

\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tikzpicture}
\tikzsetfigurename{language_cpu_inceptionv3_tensorflow}
\begin{axis}[
    ymajorgrids=true,
    grid style=dashed,
	ybar interval=0.7,
	xlabel=(b) Normalized CPU Latency.,
	font=\sffamily,
	enlargelimits=0.05,
	tick label style={font=\footnotesize},
	label style={font=\small},
    legend columns=5,
	width=0.8\linewidth,
    height=0.2\linewidth,
    axis x line*=bottom,
    axis y line=left,
    legend style={
    at={(0,0)},anchor=north west,at={(axis description cs:0.16,1.3)},
    font=\sffamily\footnotesize,fill=none,draw=none},
	cycle list name=Dark2-8,
	every axis plot/.append style={fill,draw=none,no markers},
	symbolic x coords = {1,2,4,8,16,32,999},
    xtick=data,
    bar shift=0pt,
    bar width = 10pt,
    ymin=0,
    legend image code/.code={%
        \draw[#1, draw=none] (0cm,-0.1cm) rectangle (0.2cm,0.1cm);
    },  
]
	\addplot[plotcolor1] table [x index=0,y index=4] {language_cpu_inceptionv3_tensorflow.dat};
	\addlegendentry{C++}

	
	\addplot[plotcolor3] table [x index=0,y index=5] {language_cpu_inceptionv3_tensorflow.dat};
	\addlegendentry{NumPy} 
	
	\addplot[plotcolor4] table [x index=0,y index=6] {language_cpu_inceptionv3_tensorflow.dat};
	\addlegendentry{Python}
	
        
\end{axis}
\end{tikzpicture} 
\vspace{-0.1in}
\label{fig:eval_cpu_language}
\end{subfigure}


==> latex_figures/fig_language_gpu.tex <==


 

\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{tikzpicture}
\tikzsetfigurename{language_gpu_inceptionv3_tensorflow}
\begin{axis}[
    ymajorgrids=true,
    grid style=dashed,
	ybar interval=0.7,
	xlabel=(b) Normalized GPU Latency.,
	font=\sffamily,
	enlargelimits=0.05,
	tick label style={font=\footnotesize},
	label style={font=\small},
	width=0.8\linewidth,
    height=0.2\linewidth,
    axis x line*=bottom,
    axis y line=left,
	cycle list name=Dark2-8,
	every axis plot/.append style={fill,draw=none,no markers},
	symbolic x coords = {1,2,4,8,16,32,999},
    xtick=data,
    bar shift=0pt,
    bar width = 10pt,
    ymin=0,
    legend columns=5,
    legend style={
    at={(0,0)},anchor=north west,at={(axis description cs:0,1.25)},
    font=\sffamily\footnotesize,fill=none,draw=none},
    legend image code/.code={%
        \draw[#1, draw=none] (0cm,-0.1cm) rectangle (0.2cm,0.1cm);
    },  
]
	\addplot[plotcolor1] table [x index=0,y index=4] {language_gpu_inceptionv3_tensorflow.dat};

	
	\addplot[plotcolor3] table [x index=0,y index=5] {language_gpu_inceptionv3_tensorflow.dat};
	
	\addplot[plotcolor4] table [x index=0,y index=6] {language_gpu_inceptionv3_tensorflow.dat};
	
        
\end{axis}
\end{tikzpicture} 
\label{fig:eval_gpu_language}
\end{subfigure}


==> latex_tools/protobuf_style.tex <==
\usepackage{xcolor}
\usepackage{xcolor-solarized}
\usepackage{textcomp}

\newcommand{\SetProtoColorsSolarized}{
  \colorlet{proto_basic}{solarized-base00}
  \colorlet{proto_keyword}{solarized-cyan}
  \colorlet{proto_type}{solarized-cyan}
  \colorlet{proto_options}{solarized-cyan}
  \colorlet{proto_comment}{solarized-base1}
  \colorlet{proto_string}{solarized-blue}
  \colorlet{proto_number}{solarized-violet}
  \colorlet{proto_ident}{solarized-base00}
  \colorlet{proto_digits}{solarized-violet}
  \colorlet{proto_background}{solarized-base3}
}

\newcommand{\SetProtoColorsBlueish}{
  \definecolor{proto_basic}{RGB}{0,0,0}             %
  \definecolor{proto_keyword}{RGB}{0,0,255}         %
  \definecolor{proto_type}{RGB}{128,0,0}            %
  \definecolor{proto_options}{RGB}{128,0,128}       %
  \definecolor{proto_comment}{RGB}{0,128,0}         %
  \definecolor{proto_string}{RGB}{255,0,0}          %
  \definecolor{proto_number}{RGB}{108,113,196}      %
  \definecolor{proto_ident}{RGB}{0,0,0}             %
  \definecolor{proto_digits}{RGB}{0,0,128}          %
  \definecolor{proto_background}{RGB}{255,255,255}  %
}

\newcommand{\SetProtoColorsTomorrow}{
  \definecolor{proto_basic}{RGB}{0, 0, 0}          %
  \definecolor{proto_keyword}{RGB}{0,0,0}      %
  \definecolor{proto_type}{RGB}{255,0,0}        %
  \definecolor{proto_options}{RGB}{0, 0, 0}
  \definecolor{proto_comment}{RGB}{142, 144, 140}
  \definecolor{proto_string}{RGB}{0, 0, 0}        %
  \definecolor{proto_number}{RGB}{0,0,0}
  \definecolor{proto_ident}{RGB}{0,0,255}         %
  \definecolor{proto_digits}{RGB}{0,0,255}       %
  \definecolor{proto_background}{RGB}{255, 255, 255}  %
}


\SetProtoColorsTomorrow{}



\lstdefinestyle{protobuf}{
  backgroundcolor=\color{proto_background},
  basicstyle=\color{proto_basic}\fontsize{7}{7}\ttfamily,
	keywordstyle=[1]\fontsize{7}{7}\ttfamily\mdseries\color{proto_keyword},
	keywordstyle=[2]\fontsize{7}{7}\ttfamily\mdseries\color{proto_type},
	keywordstyle=[3]\fontsize{7}{7}\ttfamily\mdseries\color{proto_options},
	commentstyle= \fontsize{7}{7}\color{purple}\ttfamily\fontsize{7}{7}\ttfamily,
	stringstyle=\color{proto_string},
  identifierstyle=\color{proto_ident},
	breaklines=true,
	showstringspaces=false,
	tabsize=2,
  literate={0}{{\textcolor{proto_digits}{0}}}{1}%
           {1}{{\textcolor{proto_digits}{1}}}{1}%
           {2}{{\textcolor{proto_digits}{2}}}{1}%
           {3}{{\textcolor{proto_digits}{3}}}{1}%
           {4}{{\textcolor{proto_digits}{4}}}{1}%
           {5}{{\textcolor{proto_digits}{5}}}{1}%
           {6}{{\textcolor{proto_digits}{6}}}{1}%
           {7}{{\textcolor{proto_digits}{7}}}{1}%
           {8}{{\textcolor{proto_digits}{8}}}{1}%
           {9}{{\textcolor{proto_digits}{9}}}{1}%
           {.0}{{\textcolor{proto_digits}{.0}}}{2}%
           {.1}{{\textcolor{proto_digits}{.1}}}{2}%
           {.2}{{\textcolor{proto_digits}{.2}}}{2}%
           {.3}{{\textcolor{proto_digits}{.3}}}{2}%
           {.4}{{\textcolor{proto_digits}{.4}}}{2}%
           {.5}{{\textcolor{proto_digits}{.5}}}{2}%
           {.6}{{\textcolor{proto_digits}{.6}}}{2}%
           {.7}{{\textcolor{proto_digits}{.7}}}{2}%
           {.8}{{\textcolor{proto_digits}{.8}}}{2}%
           {.9}{{\textcolor{proto_digits}{.9}}}{2}%
           {int32}{{\textcolor{proto_type}{int32}}}{5}%
           {int64}{{\textcolor{proto_type}{int64}}}{5}%
           {uint32}{{\textcolor{proto_type}{uint32}}}{6}%
           {uint64}{{\textcolor{proto_type}{uint64}}}{6}%
           {sint32}{{\textcolor{proto_type}{sint32}}}{6}%
           {sint64}{{\textcolor{proto_type}{sint64}}}{6}%
           {fixed32}{{\textcolor{proto_type}{fixed32}}}{7}%
           {fixed64}{{\textcolor{proto_type}{fixed64}}}{7}%
           {sfixed32}{{\textcolor{proto_type}{sfixed32}}}{8}%
           {sfixed64}{{\textcolor{proto_type}{sfixed64}}}{8}%
           {java_string_check_utf8}{{%
             \textcolor{proto_options}{java_string_check_utf8}}}{2}%
           {\ }{{ }}{1},
	prebreak=\raisebox{0ex}[0ex][0ex]{\ensuremath{\hookleftarrow}},
	upquote=true,
}

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

